Does Joint Training Really Help Cascaded Speech Translation?

Currently, in speech translation, the straightforward approach - cascading a recognition system with a translation system - delivers state-of-the-art results. However, fundamental challenges such as error propagation from the automatic speech recognition system still remain. To mitigate these problems, recently, people turn their attention to direct data and propose various joint training methods. In this work, we seek to answer the question of whether joint training really helps cascaded speech translation. We review recent papers on the topic and also investigate a joint training criterion by marginalizing the transcription posterior probabilities. Our findings show that a strong cascaded baseline can diminish any improvements obtained using joint training, and we suggest alternatives to joint training. We hope this work can serve as a refresher of the current speech translation landscape, and motivate research in finding more efficient and creative ways to utilize the direct data for speech translation.

==> old_tables.tex <==
\begin{table*}[]
\centering
\begin{tabular}{l|ccc|llll}
\hline
\multirow{3}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Data}} & \multicolumn{4}{c}{\textbf{MuST-C En-De}} \\ \cline{2-8} 
 & \multirow{2}{*}{\textbf{MT}} & \multirow{2}{*}{\textbf{ASR}} & \multirow{2}{*}{\textbf{ST}} & \multicolumn{2}{c|}{\textbf{tst-HE}} & \multicolumn{2}{c}{\textbf{tst-COMMON}} \\ \cline{5-8} 
 &  &  &  & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c|}{\textbf{TER}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c}{\textbf{TER}} \\ \hline
\textbf{other works} & \textbf{} & \textbf{} & \textbf{} &  & \multicolumn{1}{l|}{} &  &  \\
cascade \cite{baharTightIntegratedEndtoEnd2021} & \checkmark & \checkmark & \textbf{} & 25.0 & \multicolumn{1}{l|}{59.2} & 25.9 & 56.2 \\
cascade \cite{xu2021stacked} & \textbf{} & \textbf{} & \checkmark & - & \multicolumn{1}{l|}{-} & 23.3 & - \\
cascade \cite{xu2021stacked} & \checkmark & \checkmark & \checkmark & - & \multicolumn{1}{l|}{-} & 28.1 & - \\
cascade \cite{inagumaESPnetSTIWSLT20212021} & \checkmark & \checkmark & - & 26.1 & \multicolumn{1}{l|}{-} & 29.4 & - \\
direct + pretraining \cite{baharTightIntegratedEndtoEnd2021} & \checkmark & \checkmark & \checkmark & 24.4 & \multicolumn{1}{l|}{59.9} & 25.1 & 56.9 \\
direct + pretraining + multi-task \cite{xu2021stacked} & \textbf{} & \textbf{} & \checkmark & - & \multicolumn{1}{l|}{-} & 25.2 & - \\
direct + pretraining + multi-task \cite{xu2021stacked} & \checkmark & \checkmark & \checkmark & - & \multicolumn{1}{l|}{-} & 28.1 & - \\
direct + KD \cite{inagumaESPnetSTIWSLT20212021} & \checkmark & \checkmark & \checkmark & 27.4 & \multicolumn{1}{l|}{-} & 30.9 & - \\
tight integrated cascade \cite{baharTightIntegratedEndtoEnd2021} & \checkmark & \checkmark & \checkmark & 26.8 & \multicolumn{1}{l|}{57.2} & 26.5 & 54.8 \\
searchable hidden intermediates \cite{dalmia2021searchable} & \textbf{} & \textbf{} & \checkmark & - & \multicolumn{1}{l|}{-} & 26.4 & - \\ 
searchable hidden intermediates + KD \cite{inagumaESPnetSTIWSLT20212021}  & \checkmark & \checkmark & \checkmark & - & \multicolumn{1}{l|}{-} & 30.8 & - \\ \hline
\textbf{this work (no fine-tuning)} & \textbf{} & \textbf{} & \textbf{} &  & \multicolumn{1}{l|}{} &  &  \\
ground-truth transcript MT & \checkmark & (\checkmark) & \textbf{} & 30.4 & \multicolumn{1}{l|}{54.0} & 32.5  &  48.9 \\
cascade & \checkmark & \checkmark & \textbf{} & 27.7 & \multicolumn{1}{l|}{57.8} & 29.0 & 53.6 \\
tight integrated cascade & \checkmark & \checkmark & \checkmark & 28.7 & \multicolumn{1}{l|}{56.1} & 29.2 & 53.5 \\
AM-Sequence & \checkmark & \checkmark & \checkmark & 28.7 & \multicolumn{1}{l|}{56.9} & 30.0 & 52.5 \\
AM-Token & \checkmark & \checkmark & \checkmark & 28.5 & \multicolumn{1}{l|}{56.8} & 29.4 & 53.6 \\
\textbf{this work (fine-tuned ASR and MT models)} & \textbf{} & \textbf{} & \textbf{} &  & \multicolumn{1}{l|}{} &  &  \\
ground-truth transcript MT& \checkmark & (\checkmark) & \textbf{} & 31.1 & \multicolumn{1}{l|}{53.2} & 33.7 & 48.2 \\
cascade & \checkmark & \checkmark & \textbf{} & 29.1 & \multicolumn{1}{l|}{56.6} & 30.5 & 52.2 \\
tight integrated cascade& \checkmark & \checkmark & \checkmark & 29.4 & \multicolumn{1}{l|}{55.9} & 30.1 & 52.5 \\
AM-Sequence & \checkmark & \checkmark & \checkmark & 29.4 & \multicolumn{1}{l|}{55.9} & 30.5 & 51.9 \\
AM-Token & \checkmark & \checkmark & \checkmark & 23.7 & \multicolumn{1}{l|}{70.1} & 23.4 & 72.1 \\\hline
\end{tabular}
\caption{Results measured in BLEU {[}\%{]} and TER {[}\%{]} on the MuST-C En-De task. (Version 1)}
\label{tab:main_results}
\end{table*}
\begin{table*}[]
\centering
\begin{tabular}{l|ccc|llll}
\hline
\multirow{3}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Data}} & \multicolumn{4}{c}{\textbf{MuST-C En-De}} \\ \cline{2-8} 
 & \multirow{2}{*}{\textbf{MT}} & \multirow{2}{*}{\textbf{ASR}} & \multirow{2}{*}{\textbf{ST}} & \multicolumn{2}{c|}{\textbf{tst-HE}} & \multicolumn{2}{c}{\textbf{tst-COMMON}} \\ \cline{5-8} 
 &  &  &  & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c|}{\textbf{TER}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c}{\textbf{TER}} \\ \hline
\textbf{other works} & \textbf{} & \textbf{} & \textbf{} &  & \multicolumn{1}{l|}{} &  &  \\
tight integrated cascade \cite{baharTightIntegratedEndtoEnd2021} & \checkmark & \checkmark & \checkmark & 7.2\% & \multicolumn{1}{l|}{3.4\%} & 2.3\% & 2.5\% \\
direct + pretraining + multi-task \cite{xu2021stacked} & \textbf{} & \textbf{} & \checkmark & - & \multicolumn{1}{l|}{-} & 8.2\% & - \\
direct + pretraining + multi-task \cite{xu2021stacked} & \checkmark & \checkmark & \checkmark & - & \multicolumn{1}{l|}{-} & 0.0\% & - \\
searchable hidden intermediates \cite{dalmia2021searchable} & \textbf{} & \textbf{} & \checkmark & - & \multicolumn{1}{l|}{-} & 13.3\% & - \\ 
searchable hidden intermediates + KD \cite{inagumaESPnetSTIWSLT20212021} & \textbf{} & \textbf{} & \checkmark & - & \multicolumn{1}{l|}{-} & 4.8\% & - \\ \hline
\textbf{this work (no fine-tuning)} & \textbf{} & \textbf{} & \textbf{} &  & \multicolumn{1}{l|}{} &  &  \\
ground-truth transcript MT & \checkmark & (\checkmark) & \textbf{} & 30.4 & \multicolumn{1}{l|}{54.0} & 32.5  &  48.9 \\
cascade & \checkmark & \checkmark & \textbf{} & 27.7 & \multicolumn{1}{l|}{57.8} & 29.0 & 53.6 \\
tight integrated cascade & \checkmark & \checkmark & \checkmark & 28.7 & \multicolumn{1}{l|}{56.1} & 29.2 & 53.5 \\
AM-Sequence & \checkmark & \checkmark & \checkmark & 28.7 & \multicolumn{1}{l|}{56.9} & 30.0 & 52.5 \\
AM-Token & \checkmark & \checkmark & \checkmark & 28.5 & \multicolumn{1}{l|}{56.8} & 29.4 & 53.6 \\
\textbf{this work (fine-tuned ASR and MT models)} & \textbf{} & \textbf{} & \textbf{} &  & \multicolumn{1}{l|}{} &  &  \\
ground-truth transcript MT& \checkmark & (\checkmark) & \textbf{} & 31.1 & \multicolumn{1}{l|}{53.2} & 33.7 & 48.2 \\
cascade & \checkmark & \checkmark & \textbf{} & 29.1 & \multicolumn{1}{l|}{56.6} & 30.5 & 52.2 \\
tight integrated cascade& \checkmark & \checkmark & \checkmark & 29.4 & \multicolumn{1}{l|}{55.9} & 30.1 & 52.5 \\
AM-Sequence & \checkmark & \checkmark & \checkmark & 29.4 & \multicolumn{1}{l|}{55.9} & 30.5 & 51.9 \\
AM-Token & \checkmark & \checkmark & \checkmark & 23.7 & \multicolumn{1}{l|}{70.1} & 23.4 & 72.1 \\\hline
\end{tabular}
\caption{Relative improvements on the MuST-C En-De task. (Version 3: relative improvements). \cite{dalmia2021searchable} do not provide baseline cascade results so I take this number from \cite{xu2021stacked}.}
\label{tab:main_results}
\end{table*}









\begin{table*}[!th]
\centering
\begin{tabular}{l|ccc|llll}
\hline
\multirow{3}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Data}} & \multicolumn{4}{c}{\textbf{MuST-C En-De}} \\ \cline{2-8} 
 & \multirow{2}{*}{\textbf{MT}} & \multirow{2}{*}{\textbf{ASR}} & \multirow{2}{*}{\textbf{ST}} & \multicolumn{2}{c|}{\textbf{tst-HE}} & \multicolumn{2}{c}{\textbf{tst-COMMON}} \\ \cline{5-8} 
 &  &  &  & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c|}{\textbf{TER}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c}{\textbf{TER}} \\ \hline
\citet{baharTightIntegratedEndtoEnd2021} & \textbf{} & \textbf{} & \textbf{} &  & \multicolumn{1}{l|}{} &  &  \\
cascade & \checkmark & \checkmark & \textbf{} & 25.0 & \multicolumn{1}{l|}{59.2} & 25.9 & 56.2 \\
direct + pretraining & \checkmark & \checkmark & \checkmark & 24.4 & \multicolumn{1}{l|}{59.9} & 25.1 & 56.9 \\
tight integrated cascade & \checkmark & \checkmark & \checkmark & 26.8 & \multicolumn{1}{l|}{57.2} & 26.5 & 54.8 \\ \hline
\citet{xu2021stacked} & \textbf{} & \textbf{} & \textbf{} &  & \multicolumn{1}{l|}{} &  &  \\
cascade & \textbf{} & \textbf{} & \checkmark & - & \multicolumn{1}{l|}{-} & 23.3 & - \\
cascade & \checkmark & \checkmark & \checkmark & - & \multicolumn{1}{l|}{-} & 28.1 & - \\
direct + pretraining + multi-task & \textbf{} & \textbf{} & \checkmark & - & \multicolumn{1}{l|}{-} & 25.2 & - \\
direct + pretraining + multi-task & \checkmark & \checkmark & \checkmark & - & \multicolumn{1}{l|}{-} & 28.1 & - \\ \hline
\citet{dalmia2021searchable} & \textbf{} & \textbf{} & \textbf{} &  & \multicolumn{1}{l|}{} &  &  \\
searchable hidden intermediates & \textbf{} & \textbf{} & \checkmark & - & \multicolumn{1}{l|}{-} & 26.4 & - \\ \hline
\citet{inagumaESPnetSTIWSLT20212021} & \textbf{} & \textbf{} & \textbf{} &  & \multicolumn{1}{l|}{} &  &  \\
cascade & \checkmark & \checkmark & - & 26.1 & \multicolumn{1}{l|}{-} & 29.4 & - \\
direct + KD & \checkmark & \checkmark & \checkmark & 27.4 & \multicolumn{1}{l|}{-} & 30.9 & - \\
searchable hidden intermediates + KD  & \checkmark & \checkmark & \checkmark & - & \multicolumn{1}{l|}{-} & 30.8 & - \\ \hline
\textbf{this work (no fine-tuning)} & \textbf{} & \textbf{} & \textbf{} &  & \multicolumn{1}{l|}{} &  &  \\
ground-truth transcript MT & \checkmark & (\checkmark) & \textbf{} & 30.4 & \multicolumn{1}{l|}{54.0} & 32.5  &  48.9 \\
cascade & \checkmark & \checkmark & \textbf{} & 27.7 & \multicolumn{1}{l|}{57.8} & 29.0 & 53.6 \\
tight integrated cascade & \checkmark & \checkmark & \checkmark & 28.7 & \multicolumn{1}{l|}{56.1} & 29.2 & 53.5 \\
AM-Sequence & \checkmark & \checkmark & \checkmark & 28.7 & \multicolumn{1}{l|}{56.9} & 30.0 & 52.5 \\
AM-Sequence (without joint training) & \checkmark & \checkmark &  & 28.2 & \multicolumn{1}{l|}{57.1} & 29.4 & 53.1\\
AM-Token & \checkmark & \checkmark & \checkmark & 28.5 & \multicolumn{1}{l|}{56.8} & 29.4 & 53.6 \\
\textbf{this work (fine-tuned ASR and MT models)} & \textbf{} & \textbf{} & \textbf{} &  & \multicolumn{1}{l|}{} &  &  \\
ground-truth transcript MT& \checkmark & (\checkmark) & \textbf{} & 31.1 & \multicolumn{1}{l|}{53.2} & 33.7 & 48.2 \\
cascade & \checkmark & \checkmark & \textbf{} & 29.1 & \multicolumn{1}{l|}{56.6} & 30.5 & 52.2 \\
tight integrated cascade& \checkmark & \checkmark & \checkmark & 29.4 & \multicolumn{1}{l|}{55.9} & 30.1 & 52.5 \\
AM-Sequence & \checkmark & \checkmark & \checkmark & 29.4 & \multicolumn{1}{l|}{55.9} & 30.5 & 51.9 \\
AM-Sequence (without joint training) & \checkmark & \checkmark & \textbf{ } & 29.4 & \multicolumn{1}{l|}{56.4} & 30.8 & 51.9 \\
AM-Token & \checkmark & \checkmark & \checkmark & 23.7 & \multicolumn{1}{l|}{70.1} & 23.4 & 72.1 \\\hline
\end{tabular}
\caption{Results measured in BLEU {[}\%{]} and TER {[}\%{]} on the MuST-C En-De task. (Version 2: separate by authors)}
\label{tab:main_results}
\end{table*}
